Application of interpretable machine learning for cross-diagnostic inference on the ST40 spherical tokamak

Machine learning models are exceptionally effective in capturing complex non-linear relationships of high-dimensional datasets and making accurate predictions. However, their intrinsic ``black-box'' nature makes it difficult to interpret them or guarantee ``safe behavior'' when deployed in high-risk applications such as feedback control, healthcare and finance. This drawback acts as a significant barrier to their wider application across many scientific and industrial domains where the interpretability of the model predictions is as important as accuracy. Leveraging the latest developments in interpretable machine learning, we develop a method to parameterise ``black-box'' models, effectively transforming them into ``grey-box'' models. We apply this approach to plasma diagnostics by creating a parameterised synthetic Soft X-Ray imaging $-$ Thomson Scattering diagnostic, which predicts high temporal resolution electron temperature and density profiles from the measured soft X-ray emission. The ``grey-box'' model predictions are benchmarked against the trained ``black-box'' models as well as a diverse range of plasma conditions. Our model-agnostic approach can be applied to various machine learning architectures, enabling direct comparisons of model interpretations.

==> figures.tex <==

\begin{figure*}
\includegraphics[width=\textwidth]{figures/shap_model_comparison.PNG}
\put(-460,60){\rotatebox{90}{$\delta n_e(\textrm{Los})\times 10^{20}$ [$m^{-3}$]  contribution from input feature }}\put(-300,-10){Normalised soft x-ray emission $\epsilon$}
\caption{\label{fig:shape_ml_comparison} Computed SHAP values for the training dataset for feed-forward neural net model (FFNN), random forest (RF) and Gaussian Process Regression model (GPR).}
\end{figure*}


\begin{figure*}
%\includegraphics[width=\textwidth]{figures/ale_vs_ml_vs_ts_ne.png}
%\includegraphics[width=\textwidth]{figures/ale_vs_ml_vs_ts_te.png}
\includegraphics[width=\textwidth]{figures/ale_vs_ml_combined.png}
\put(-420,300){(a)}
\put(-420,150){(b)}
\caption{\label{fig:ale_ml_ts_predictions} Plasma shot 11574. (a) Time dependent density trace of core line of sight. The shaded red region indicates where the TS beam suffers from transient pointing instability due to mechanical vibrations. The diamond tickers show the measured Thomson scattering density. The solid lines show the predicted time dependent density of the same TS line of sight using the parametrised ALE model as well as the original neural network. (b) Time dependent temperature trace of core line of sight. The shaded red region between 25ms and 50ms is where the TS diagnostic experiences mechanical vibrations during the merging compression startup which affect the collection of scattered light resulting in a systematic dip in the density and an increase in error estimation of the temperature. However, the measured SXR input emission is robust to mechanical vibrations and as a result the model does not show it the predicted temperature and density estimates.\textcolor{red}{TP: Include ECE data and if we have SMM data on a separate plot for validation}}
\end{figure*}

\begin{figure*}
%\includegraphics[width=\textwidth]{figures/ale_vs_ml_vs_ts_ne.png}
%\includegraphics[width=\textwidth]{figures/ale_vs_ml_vs_ts_te.png}
\includegraphics[width=\textwidth]{figures/ale_gpr.png}
\put(-440,360){(a)}
\put(-440,180){(b)}
\caption{\label{fig:ale_gpr_predictions} Plasma shot 11574. (a) Time dependent density trace of core line of sight. The diamond tickers show the measured Thomson scattering density. The solid lines show the predicted time dependent density of the same TS line of sight using the parametrised ALE model as well as the original GPR prediction. (b) Time dependent temperature trace of core line of sight. As demonstrated with FFNN results in Fig.~\ref{fig:ale_ml_ts_predictions}, the measured SXR input emission is robust to mechanical vibrations and as a result the GPR model does not show it in the predicted temperature and density estimates.\textcolor{red}{TP: Include ECE data and if we have SMM data on a separate plot for validation. Also include uncertainty estimate in the GPR model.}.}
\end{figure*}

\begin{figure*}[t] 
\centering
 \makebox[\textwidth]{\includegraphics[width=.7\paperwidth]{figures/ml_predictions_for_different_plasma_shots.png}}
\caption{Model performance across different plasma pulses. Top to bottom: 11032, 11089, 11378, 11519, 11559, 11560, 11574. For plasma scenario details refere to Table~\ref{tab:plasma_scenarios}}
\label{fig:model_comparisons}
\end{figure*}
